Scalar curvature, metric degenerations and the static vacuum Einstein equations on 3-manifolds, II

This paper is a continuation of I, (same title), and is concerned with the existence, regularity and degeneration of metrics minimizing natural curvature functionals on the space of metrics on 3-manifolds. The functionals chosen are designed to be optimal w.r.t. the issue of geometrization of the underlying 3-manifold, in the sense of Thurston. Two of the main results are Theorems B and C, in comparison with Theorem A of I.

==> ref.tex <==
\bibliographystyle{plain}
\begin{thebibliography}{WWW}

 
\footnotesize 
\bibitem[Ab]{Ab} U. Abresch,
        Lower curvature bounds, Toponogov's theorem, and bounded topology,
        Ann. Sci. Ecole Norm. Sup., vol. 18, (1985), 651-670. 

\bibitem[Ad]{Ad} R. Adams,
	Sobolev Spaces,
	Academic Press, New York, (1975).

\bibitem[AnI]{AnI} M. Anderson,  
        Scalar curvature, metric degenerations and 
        the static vacuum Einstein equations on 3-manifolds, I, 
        Geom. \& Funct. Analysis, vol. 9, (1999), 855-967. 

\bibitem[An2]{An2} \_\_\_\_\_\_,  
	Scalar curvature and geometrization conjectures for 3-manifolds,
	Comparison Geometry, MSRI Publ., vol. 30, (1997), 49-82.

\bibitem[An3]{An3} \_\_\_\_\_\_, 
        Extrema of curvature functionals on the space of metrics 
	on 3-manifolds,
	Calc. of Var. \& P.D.E., vol. 5:3, (1997), 199-269.

\bibitem[An4]{An4} \_\_\_\_\_\_,         
        Extrema of curvature functionals on the space of metrics 
on 3-manifolds, II, 
        Calc. of Var. \& P.D.E., vol. 11, (2000).

\bibitem[An5]{An5} \_\_\_\_\_\_,  
        On the structure of solutions to the static vacuum Einstein equations,
        Annales Henri Poincar\'e, vol. 1, (2000), (to appear).

\bibitem[An6]{An6} \_\_\_\_\_\_,
	Scalar curvature and the existence of geometric structures 
on 3-manifolds, I,
	(preprint, Stony Brook, Sept. 2000).        

	The papers above are
        available at: http://www.math.sunysb.edu/ $\sim $ anderson/

\bibitem[BKN]{BKN} S. Bando, A. Kasue and H. Nakajima,
        On a construction of coordinates at infinity on manifolds with fast
        curvature decay and maximal volume growth,
        Invent. Math., vol. 97, (1989), 313-349.

\bibitem[B]{B} A. Besse, 
       Einstein Manifolds, Ergebnisse der Mathematik, 3. Folge, Band 10,
       Springer Verlag, New York (1987).

\bibitem[CG1]{CG1} J. Cheeger and M. Gromov, 
      Collapsing Riemannian manifolds while keeping their curvature bounded I, 
      Jour. Diff. Geom. vol. 23, (1986), 309-346.

\bibitem[CG2]{CG2} \_\_\_\_\_\_,  
      Collapsing Riemannian manifolds while keeping their curvature bounded II,       Jour. Diff. Geom. vol. 32., (1990), 269-298.

\bibitem[CY]{CY} S.Y. Cheng and S.T. Yau, 
	Differential equations on Riemannian manifolds and their geometric applications,
	Comm. Pure Appl. Math., vol. 28, (1975), 333-354.

\bibitem[EK]{EK} J. Ehlers and W. Kundt,
	Exact solutions of the gravitational field equations, in Gravitation: An Intro. to Current Research, (L. Witten, Ed.), J. Wiley, N.Y., (1962), 49-101.

\bibitem[Fu]{Fu} K. Fukaya, 
     Hausdorff convergence of Riemannian manifolds and its applications,
     in Adv. Stud. in Pure Math, vol. 18-I, Recent Topics in Diff. and Anal. Geom., (T. Ochiai, Ed.), Kinokuniya, Tokyo, (1990), 143-238.

 
\bibitem[GT]{GT} D. Gilbarg and N. Trudinger, 
     Elliptic Partial Differential Equations of the Second Order,
     2$^{\rm nd}$ Edition, Springer Verlag, New York, 1983.

\bibitem[Gr1]{Gr1} M. Gromov, 
    Structures M\'etriques pour les Vari\'et\'es Riemanniennes,
    Cedic-Fernand/Nathan, Paris (1981).

\bibitem[Gr2]{Gr2} \_\_\_\_\_\_,
	Large Riemannian manifolds, 
	in Curv. and Top. of Riemannian Manifolds, Lecture Notes in Math., vol. 1201, Springer Verlag, (1986), 108-121.


\bibitem[GL1]{GL1} M. Gromov and H.B. Lawson, Jr., 
    The classification of simply connected manifolds of positive
    scalar curvature,
    Annals of Math., vol. 111, (1980), 423-434.

\bibitem[GL2]{GL2} \_\_\_\_\_\_, 
     Positive scalar curvature and the Dirac operator on complete 
     Riemannian manifolds,
     Publ. Math. I.H.E.S., vol. 56, (1983), 83-196.

\bibitem[Gu]{Gu} M. Gursky,
	Compactness of conformal metrics with integral bounds on curvature,
	Duke Math. Jour., vol. 72, (1993), 339-367.

\bibitem[H]{H} J. Hempel,
      3-Manifolds,
      Annals of Math. Studies, vol. 86, Princeton Univ. Press, Princeton,
      (1976).

\bibitem[J]{J} W.H. Jaco, Lectures on Three-Manifold Topology
      C.B.M.S., vol. 43, Amer. Math. Soc., (1980).

\bibitem[K]{K} O. Kobayashi, Scalar curvature of a metric of unit volume,
                 Math. Annalen, vol. 279, (1987), 253-265.

\bibitem[LP]{LP} J. Lee and T. Parker, 
        The Yamabe problem, Bull. Amer. Math. Soc.,
        17:1, (1987), 37-91.

\bibitem[La]{La} F. Lamontagne,
	A critical metric for the $L^{2}$ norm of the curvature tensor on $S^{3}$,
	Proc. Amer. Math. Soc., vol. 126, (1998), 589-593.

\bibitem[Lu]{Lu} X.-d. Liu,
        Ball covering on manifolds with non-negative Ricci curvature
        near infinity,
        Proc. Symp. Pure Math., A.M.S., vol. 54:3, (1993), 459-464.

\bibitem[MTW]{MTW} C.W. Misner, K.S. Thorne and J.A. Wheeler, 
        Gravitation,
        W.H. Freeman, New York, (1973).

\bibitem[Mo]{Mo} C.B. Morrey, Jr,
        Multiple Integrals in the Calculus of Variations,
        Grundlehren Series, Vol. 130, Springer Verlag, New York, (1966).

\bibitem[O]{O} P. Orlik, Seifert Manifolds,
        Lect. Notes in Math., vol. 291,
        Springer Verlag, New York, (1972).

\bibitem[R]{R} X. Rong, 
        The limiting eta invariant of collapsed 3-manifolds,
        Jour. Diff. Geom., vol. 37, (1993), 535-568.

\bibitem[S]{S} R. Schoen, 
         Variational theory for the total scalar curvature functional 
         for Riemannian metrics and related topics, 
        Lect. Notes Math. vol. 1365, Springer Verlag, Berlin, (1987), 120-154.

\bibitem[SY1]{SY1} R. Schoen and S.T. Yau, 
        On the proof of the positive mass conjecture in general relativity,
        Comm. Math. Phys., vol. 65, (1979), 45-76.

\bibitem[SY2]{SY2} \_\_\_\_\_\_,
        On the structure of manifolds with positive scalar curvature,
        Manuscripta Math., vol. 28, (1979), 159-183.

\bibitem[SY3]{SY3} \_\_\_\_\_\_,
        Complete three-dimensional manifolds with positive Ricci curvature
        and scalar curvature,
        Seminar on Diff. Geom, Ann. of Math. Stud., vol. 102, Princeton Univ.
        Press, (1982), 209-227.

\bibitem[St]{St} P. Scott, 
        The geometries of 3-manifolds,
        Bull. London Math. Soc., vol. 15, (1983), 401-487.

\bibitem[So]{So} T. Soma, 
        The Gromov invariant of links,
        Invent. Math., vol. 64, (1981), 445-454.

\bibitem[Th]{Th} W. Thurston,
	Three dimensional manifolds, Kleinian groups and hyperbolic geometry, 
	Bull. Amer. Math. Soc, vol. 6, (1982), 357-381.

\bibitem[Tr]{Tr} F. Treves, 
       Basic Linear Partial Differential Equations,
       Academic Press, New York, (1975).

\bibitem[Wd]{Wd} R.M. Wald,
       General Relativity,
       Univ. of Chicago Press, Chicago, (1984).

\bibitem[Wa]{Wa} F. Waldhausen, 
       Eine Klasse von 3-dimensionalen Mannifaltigkeiten I,II,
       Invent. Math., vol 3, (1967), 308-333, and vol. 4, (1967), 87-117.

\end{thebibliography}

